Robust Lower Bounds for Graph Problems in the Blackboard Model of Communication

We give lower bounds on the communication complexity of graph problems in the multi-party blackboard model. In this model, the edges of an $n$-vertex input graph are partitioned among $k$ parties, who communicate solely by writing messages on a shared blackboard that is visible to every party. We show that any non-trivial graph problem on $n$-vertex graphs has blackboard communication complexity $\Omega(n)$ bits, even if the edges of the input graph are randomly assigned to the $k$ parties. We say that a graph problem is non-trivial if the output cannot be computed in a model where every party holds at most one edge and no communication is allowed. Our lower bound thus holds for essentially all key graph problems relevant to distributed computing, including Maximal Independent Set (MIS), Maximal Matching, ($\Delta+1$)-coloring, and Dominating Set. In many cases, e.g., MIS, Maximal Matching, and $(\Delta+1)$-coloring, our lower bounds are optimal, up to poly-logarithmic factors.

==> silent.tex <==
\section{Silent Algorithms and Non-Trivial Problems} \label{sec:silent}


We say that a deterministic algorithm for a problem $P$ is \emph{silent} if the algorithm solves $P$ in the $\local$ model with no communication rounds.
A problem is \emph{non-trivial} if it admits no silent algorithms.

\begin{lemma}\label{lem:randNonTrivial}
	Let $P$ be a non-trivial problem. Then there exists a positive $\epsilon = \epsilon(P)$ such that
	there is no randomized algorithm with expected time complexity $o(1)$ which solves $P$ 
	with error probability at most $\epsilon$ in the $\local$ model.
\end{lemma}
\begin{proof}
	Let $t = t(P)$ be the minimum natural number so that any deterministic silent algorithm fails to solve $P$ on every input $t$-vertex graph. Since $P$ is a non-trivial problem, such $t$ exists.
	
	Let $\epsilon = 2^{-\left( {t \choose 2} + 2 \right) }$ and suppose towards the contradiction there
	exists a randomized algorithms $A$ with expected time complexity $o(1)$ that solves $P$ in the $\local$ model with error probability at most $\epsilon$.
	The assumption on the time complexity of $A$ implies that the probability that the running time of $A$ is
	0 is $1 - o(1)$. We now construct a new algorithm $A'$ that returns an arbitrary output if the running time of $A$ is larger than 0, and executes $A$, otherwise. The running time of $A'$ is always 0 and the error probability is at most $\epsilon + o(1)$.
	
	The latter together with Yao's lemma \cite{yao1977probabilistic} imply that for any distribution over the input $t$-vertex graphs, there exists a deterministic algorithm that solves $P$ in the $\local$ model in 0 rounds with distributional error at most $2\epsilon + o(1)$. Let $B$ be such an algorithm for the uniform distribution. Since the probability of every input graph is $2^{-{t \choose 2}} > 2\epsilon + o(1)$, it follows that $B$ correctly solves $P$ on every input $t$-vertex graph, a contradiction.
\end{proof}


\subsection{Combinatorial Lower Bounds for Distributed Symmetry Breaking Problems}

By definition, any non-zero lower bound on the time complexity in the $\local$ model for a problem implies that the problem is non-trivial. Hence, \textsc{Minimal Vertex Cover}, \textsc{Maximal Independent Set}, \textsc{Maximal Matching}, \textsc{Minimum Dominating Set}, and \textsc{Minimum Connected Dominating Set} are non-trivial problems \cite{kuhn2016local}.

In this section we show that for every $t \geq 2$ the \textsc{$t$-Ruling Set} problem is also non-trivial.
To do this, let us fix $k$ and assume that inputs are $k$-vertex graphs with vertices $v_1, v_2, \ldots, v_k$, where the input of player $i$ is vertex $v_i$ together with its neighbourhood $N(v_i)$. 
Let $A$ be an algorithm for the \textsc{$t$-Ruling Set} problem. For two distinct players $p,q \in [k]$ we say that \emph{player $q$ dominates player $p$ (with respect to $A$)}, and denote this by $p <_A q$, if for any input graph $G$ vertex $v_p$ is not selected to the solution by player $p$ whenever $v_p$ is adjacent to $v_q$ in $G$. A key ingredient of our proof is the fact that the domination relation $<_A$ is a strict total order if $A$ is a silent algorithm.

\begin{lemma}\label{lem:totalOrder}
	For any silent algorithm $A$, the domination relation $<_A$ is a strict total order over $\{v_1, v_2, \ldots, v_t\}$.
\end{lemma}
\begin{proof}
	We will prove the statement  by showing that $<_A$ is  semiconnex, asymmetric, and transitive relation.
	To show that $<_A$ is semiconnex, assume to the contrary that there exist two distinct players $p,q \in[k]$
	such that neither $p <_A q$, nor $q <_A p$ holds. Since  $p \nless_A q$, there exists a graph $G_1$ such that 
	$(p,q) \in E(G)$ and $v_p$ is selected to the solution by player $p$. Similarly, since $q \nless_A p$, there exists
	a graph $G_2$ such that $(p,q) \in E(G_2)$ and $v_q$ is selected to the solution by player $q$.
	Since the output of a silent algorithm at a vertex $v$ is determined by the input of $v$, i.e. by $v$ and its
	neighbourhood $N(v)$,  
	for any input graph $H$ with $N_H(v_p) = N_{G_1}(v_p)$ and
	$N_H(v_q) = N_{G_2}(v_q)$, both $v_p$ and $v_q$ are selected by their players. But this contradicts
	the fact that any $t$-ruling set is an independent set.
	
	Now, to show that $<_A$ is asymmetric, we assume to the contrary that both $p <_A q$ and $q <_A p$ hold for some
	pair $p,q \in [k]$ of distinct players. Then it follows from the definition of $<_A$ that for any input graph in which $\{v_p, v_q\}$ 
	is a connected component, none of $v_p$ and $v_q$ is selected to the solution, which is not possible
	as any $t$-ruling set should contain at least one vertex from every connected component.
	
	Finally, to show that $<_A$ is transitive, assume to the contrary that there exist three pairwise distinct players $p,q,r$
	such that $p <_A q$, $q <_A r$, but $r <_A p$. Then for any graph $G$ in which $\{ v_p, v_q, v_r \}$ is a connected component and a clique, none of the three vertices is selected to the solution, which is a contradiction as before.
\end{proof} 



\begin{theorem}\label{th:noSilent}
	For any $t \geq 2$, the \textsc{$t$-Ruling Set} problem is non-trivial.
\end{theorem}
\begin{proof}
	Suppose, for the sake of contradiction, that there exists a silent algorithm $A$ which solves \textsc{$t$-Ruling Set} in the $\local$ model on every $k$-vertex graph, where $k=t+2$.
	By Lemma \ref{lem:totalOrder}, the relation $<_A$ is a strict total order over $\{v_1, v_2, \ldots, v_k\}$.
	Without loss of generality, assume $v_1 <_A v_2 <_A \ldots <_A v_{k-1} <_A v_k$.
	Let the input graph $G$ be the path on vertices $v_1, v_2, \ldots, v_k$ such that $(v_i,v_{i+1}) \in E(G)$ for every $i \in [k-1]$.
	Then, by the definition of $<_A$, none of $v_1, v_2, \ldots, v_{k-1}$ is selected to the solution.
	This is not possible, as $v_k$ alone does not form a $t$-ruling set in $G$. This contradiction completes the proof.
\end{proof}








==> tools.tex <==
\section{Tools from Information Theory}

\begin{definition} \label{def:totalvariation}
  Let $X$ be a discrete random variable and consider two probability distributions $p(X)$ and $q(X)$.
  The \emph{total variation distance} between $p(X)$ and $q(X)$ is defined as
  \[
    \delta_{TV} \lb( p(X), q(X) \rb) = \frac{1}{2} \sum_{x}^{} \lb| p(x) - q(x) \rb|.
  \]
\end{definition}

\begin{definition} \label{def:divergence}
  Let $X$ be a discrete random variable.
  For probability distributions $p(X)$ and $q(X)$, the \emph{Kullback–Leibler divergence from $q(X)$ to $p(X)$ (measured in bits)} is defined as
  \begin{align}
    \DD \lb[ p(X) \parallel q(X) \rb]
    =
    \sum_{x} p(x) \log \frac{p(x)}{q(x)}.
  \end{align}
\end{definition}

\begin{theorem}[Pinsker's Inequality~\cite{pinsker1964information}] \label{thm:pinsker}
  Let $X$ be a random variable. For any two probability distributions $p(X)$ and $q(X)$, it holds that
  \[
    \delta_{TV}\lb(p(X),q(X)\rb) \le \sqrt{\frac{\log 2}{2} \DD \lb[ p(X) \parallel q(X) \rb]}.
  \]
\end{theorem}


